Shabari: Delayed Decision-Making for Faster and Efficient Serverless Functions

Serverless computing relieves developers from the burden of resource management, thus providing ease-of-use to the users and the opportunity to optimize resource utilization for the providers. However, today's serverless systems lack performance guarantees for function invocations, thus limiting support for performance-critical applications: we observed severe performance variability (up to 6x). Providers lack visibility into user functions and hence find it challenging to right-size them: we observed heavy resource underutilization (up to 80%). To understand the causes behind the performance variability and underutilization, we conducted a measurement study of commonly deployed serverless functions and learned that the function performance and resource utilization depend crucially on function semantics and inputs. Our key insight is to delay making resource allocation decisions until after the function inputs are available. We introduce Shabari, a resource management framework for serverless systems that makes decisions as late as possible to right-size each invocation to meet functions' performance objectives (SLOs) and improve resource utilization. Shabari uses an online learning agent to right-size each function invocation based on the features of the function input and makes cold-start-aware scheduling decisions. For a range of serverless functions and inputs, Shabari reduces SLO violations by 11-73% while not wasting any vCPUs and reducing wasted memory by 64-94% in the median case, compared to state-of-the-art systems, including Aquatope, Parrotfish, and Cypress.

==> 10_acknowledgements.tex <==
\section{Acknowledgements}
\label{sec:acknowledgements}

==> 1_0_introduction.tex <==
\section{Introduction}
\label{sec:introduction}

%To be accessible to any kind of user, 
%Serverless computing~\cite{} \neeraja{cite AWS lambda, Azure functions and Google cloud functions} relieves cloud users from the burden of resource management. %, giving providers the opportunity to optimize resource utilization.
%Currently, serverless platforms make resource allocation decisions for all future invocations \emph{as soon as} a function is registered with the platform.
%Making \emph{immediate} resource allocation decisions enables providers to plan for the future; for example, providers can maintain a pool of pre-warm containers to mitigate cold start overheads \cite{AWS-Provisioned-Concurrency}.

One of the most significant benefits of serverless computing for developers is that it requires no management. 
Developers do not need to hand-specify their resource needs: the provider makes these decisions for them and developers can focus on the application logic alone. 
However, today's serverless systems end up adversely impacting developers and providers. 
For users with performance-critical applications, such as detection of videos with indecent contents uploaded to YouTube, %or for cost-minded applications, such as personal photo organization, 
unknown resource management policies that they cannot control are a problem ~\cite{BV_ServerlessComputing, Cold-Start-Overheads}. 
On the other side, providers lack visibility into user-functions limiting their ability to make cost-performance trade-offs on behalf of the users while optimizing resource efficiency.
%\prasoon{I'm wondering if saying "lack visibility into user-functions" makes sense to say? In our system, we analyze the function and extract information from it, suggesting that we can look into user functions. Wording might confuse the reader.}

%This opacity has forced 
Today's serverless computing frameworks launch the same sized container for all future invocations of a function, based on the size chosen at the time of a function's registration.
%Today's serverless computing frameworks make resource allocation decisions for all future invocations \emph{as soon as} a function is registered with the platform~\cite{}.\neeraja{cite}. 
Making this resource allocation decision \emph{early} in the life-cycle of a function enables providers to plan for the future; for example, providers can maintain a pool of pre-warm containers to mitigate cold start overheads \cite{AWS-Provisioned-Concurrency}. 
%\emph{immediate} resource allocation decisions enables providers to plan for the future; for example, providers can maintain a pool of pre-warm containers to mitigate cold start overheads \cite{AWS-Provisioned-Concurrency}. 
%To mitigate this opacity, most frameworks ~\cite{AWSLAMBDA, GoogleCloudFunctions, ApacheOpenWhisk} provide a single knob, the memory size of the container, that the developer can set. This parameter is intended to give users control on resource management and providers visibility into user functions. 
%However, even with this additional input, existing resource management policies have had to resort to simplifying assumptions to make \emph{early} decisions:
However, both the users and the providers suffer due to such early decision-making policies for functions:

%However, determining the resource needs of future invocations \emph{immediately} upon function registration is difficult to do with little information.
%To make such early decisions,  AWS Lambda~\cite{} exposes a single knob, the memory limit, for user to set.
%However, several studies show that providers continue to face poor resource utilization (less than 30\% of allocated resources are utilized) []\neeraja{cite}.
%Meanwhile, users with latency sensitive applications often face several service-level objective (SLO) violations []\neeraja{cite}.
%Even with the memory limit, providers lack the information required to make accurate resource allocations for future invocations. 
%Hence, existing policies have had to resort to simplifying assumptions to make \emph{early} resource allocation decisions:


% Serverless computing has been widely adopted in the past 7 years due to its fine-grained, pay-per-use model and its accessibility to any kind of user. 
% With serverless computing, the burden of resource management has shifted from the developer to the cloud provider. 
% Hence, developers can focus solely on writing their business logic while cloud providers have the opportunity to optimize resource utilization. 

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[scale=0.25]{figures/intro_plots/memory_size_duration_modified-1.png}
         %\vspace{-7mm}
         \caption{\small{Slowdown w.r.t. the best runtime across mem sizes for 100 invocations of a video transcoding function.}}% The y-axis shows the slowdown compared with the best duration observed for the given input across memory sizes.}}
         \label{fig:memory_size_duration_modified}
     \end{subfigure}
     %\hfill
     \hspace{5mm}
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[scale=0.25]{figures/intro_plots/memSize_maxMemoryUsed_new_modified-1.png}
         %\vspace{-7mm}
         \caption{\small{Maximum mem utilized vs. allocated across 100 runs of the video transcoding function (from Fig.~\ref{fig:memory_size_duration_modified}).}}%, across different memory sizes allocated.}}
         \label{fig:memSize_maxMemoryUsed_new_modified}
     \end{subfigure}
     \vspace{-2mm}
        \caption{\small{Characterizing functions with respect to the resources allocated, utilized, and performance observed.}}
        \label{fig:three graphs}
        \vspace{-4mm}
\end{figure}

% Upon function registration, serverless platforms \emph{immediately} determine the resource allocation for all future invocations of the function.
% Resource allocation decisions are made \emph{as soon as possible} in an attempt to mitigate the cold start overheads of creating function containers on the critical path of an invocation.
% With these early allocation decisions, providers pre-warm a number of containers, usually specified by the develoepr [].

% Determining the resource needs of future invocations upon function registration is difficult to do with little information.
% Hence, in an attempt to gain some insight into function needs, providers expose a single knob, the memory limit, that the user sets ~\cite{ApacheOpenWhisk}.
% However, even with this interface, several studies show that serverless providers continue to face poor resource utilization; less than 30\% of allocated resources are utilized [].
% Meanwhile, users with latency-sensitive application, such as timely detection of videos with indecent content uploaded to YouTube, often face several service-level objective (SLO) violations []. With a lack of insight into future invocation needs, providers have to resort to simplifying assumptions, reflected in their resource management policies:

\noindent\textbf{1. Early and input-agnostic allocation decisions:}
Function inputs are mostly not available until invocation time. So, providers are forced to make input-agnostic resource allocation decisions.
% To allocate resources immediately upon function registration, providers are forced to ignore inputs.
Across inputs, the performance and resource utilization varies greatly, as demonstrated in Figure ~\ref{fig:three graphs}a.
% However, depending on the inputs, we observe different performance and resource utilization for the same amount of allocation.
% However, inputs submitted to the same function can have different resource needs and result in different observed performance for the same amount of resources allocated to them, as demonstrated by the spread in duration in Figure ~\ref{fig:three graphs}a.
Thus, such decisions made prematurely without considering inputs preclude optimizations, including downsizing containers for smaller inputs, which would bring significant cost benefits and improved resource utilization.
For example, if the early, function-level allocation sizes a container with 3GB of memory, and most invocation use only 1GB, the costs incurred are 2$\times$ higher for allocated but unused resources while utilization is only 33\%. \neeraja{Where is the data to support this? I thought  you were going to bring in data from your own characterization study here.}
% Allocating resources upon function registration ignores the fact that different inputs submitted to the same function might have different resource needs (as demonstrated by the spread in duration in Figure ~\ref{fig:three graphs}a).
% This precludes optimizations including downsizing containers for smaller inputs, which may bring significant cost benefits. 
% For instance, if the static, function-level allocator sizes a container with 3GB of memory, and most invocations use only 1GB, the costs incurred are 2x higher for allocated bu unused resources.
\emph{
% Hence, serverless platforms should allocate resource dynamically by considering the inputs provided per invocation
Instead, we argue for resource allocation decisions specialized to each input to a function. Hence, instead of making early resource allocation decisions, we intentionally delay these decisions until after input to an invocation is available.
}

\noindent\textbf{2. Early-binding of different resource types:}
%\kostis{Rigid coupling instead of early binding?} \neeraja{this is intentional to the new story we are going with.}
Today's serverless platforms allocate fixed-proportions of different resource types (CPU, memory) per function, thereby early-binding different resource types.
% Given today's interfaces, at function registration, providers only have knowledge about the memory requirements of a function (specified by the developer), not other resource types (e.g., compute).
 %\kostis{Maybe mention that this by design, otherwise users would have to handle resource allocation fully defeating the purpose of serverless computing.}
% Hence, to make allocations generalizable to a variety of functions, providers assume functions are both memory- and compute-intensive by allocating a proportional number of vCPUs to the developer-specified memory limit.
However, this policy assumes that functions are both memory- and compute-intensive and leads to sub-optimal allocation decisions.
For example, a compute-intensive video transcoding function wastes up to 50\% of its memory allocation (Figure ~\ref{fig:three graphs}b).
% a 3GB memory allocation to obtain more vCPUs for a compute-intensive video transcoding function wastes 50\% of its memory (Figure ~\ref{fig:three graphs}b).
% Providers use the developer-specified memory size to proportionally allocate the number of vCPUs to a function, thus tightly coupling the two types of resources together.
% However, this assumes functions are both memory- and compute-intensive.
% Tightly coupling resources may lead to suboptimal resource allocation. 
% For example, CPU intensive workloads may be allocated more memory than required (Figure ~\ref{fig:three graphs}b). 
\emph{Instead, we make allocation decisions for each resource type independently and intentionally delay making these decisions to consider the inputs.}

\noindent\textbf{3. Memory-Centric User Interface:}
%\kostis{Resource-Centric instead of memory-centric?} \neeraja{who offers anything but memory as a knob?}
As shown \neeraja{shown where?}, the memory specification entirely determines the allocation for all future invocations.
The importance of the memory size parameter and its opaque coupling to other resource types forces users to profile their function to determine the right setting.
However, as the performance and resource utilization of a function  depends significantly on its inputs, users must profile on a diverse set of inputs to ensure adequate resource availability in all cases. 
The cost of extensive profiling is prohibitive. 
% Prior work on reducing this profiling cost either assumes knowledge of the workload which is unavailable~\cite{Ernest, Cherrypick}, or ignores the input itself, which can have a large impact on many functions ~\cite{PARIS}.
Thus, users often overprovision and choose the largest memory size available (10GB for AWS Lambda, for instance), %raising their costs significantly and 
leading to underutilized resources for the provider [2]. 
\emph{Instead of the memory-centric user interface, we argue 
%and not require users to specify resource limits. 
% Instead, serverless platforms should determine the optimal resource limits per invocation
%Instead, 
for an interface to the serverless systems that is performance-centric, allowing users to specify performance needs per invocation
}. 
%\neeraja{the performance-centric interface point should come somewhere here}

\noindent\textbf{Prior Work:} 
Previous works attempt to resolve these inefficiencies.
Open-source developer tools have been created to assist developers in determining the optimal memory limit for their function ~\cite{AWSLambdaPowerTuning, ParrotFish}.
Bin-packing solutions are proposed to pack containers with invocations and improve container utilization ~\cite{cypress, golgi}.
Finally, several learning-based solutions have been proposed to predict the optimal resource allocation or execution time of invocations \neeraja{citations?}.
However, these works still operate in the regime of early decision-making, as they only address a subset of the aforementioned inefficiencies of existing resource allocation policies.
\neeraja{This prior work para didn't work for me. It doesn't convince me that existing work isn't enough. You list existing work and say they only solve one of the prev. mentioned inefficiencies without exaplaining how and which ones, etc. Go a bit deeper without being too long, of course.}
\kostis{I agree}

%\noindent\textbf{Our Key Insight:} 
\noindent\textbf{Our Work:} We argue that the root cause of poor resource utilization and function performance is that allocation decisions for invocations are made \emph{as soon as possible} without information about the invocation needs.
%\kostis{maybe ...allocation decisions are made as soon as possible at function granularity instead of specializing for individual invocation needs.}\neeraja{we aren't just talking about input-awareness anymore. the whole story is about as late as possible, so no need to mention function-granularity here.}
%Hence, we revisit the time at which resource allocation decisions are made.
Through our measurement study, %We extensively characterize 12 commonly deployed serverless functions covering a wide range of applications.
we find that input properties, not just limited to input size, and function semantics greatly affect function execution time and resource utilization.
Moreover, we show the importance of making independent allocations for each resource type (CPU, memory) to achieve high utilization.

% Unlike previous work, we show that both properties of inputs, not just limited to input size, and function semantics greatly fluctuate function execution time and resource utilization.
% Moreover, we show the importance of making resource allocations per resource type to meet invocation SLOs while achieving high resource utilization.

%Our characterization presents tangible design requirements for serverless resource management.
%To meet these design requirements, we argue that optimal resource allocation decisions \emph{should be made at the time of an invocation}.
We build \system, a resource management framework for serverless systems that makes resource allocation decisions \textbf{A}s \textbf{L}ate \textbf{A}s \textbf{P}ossible to account for the needs of each function invocation.
{\system} introduces a performance-centric interface that allows users to specify their SLOs per invocation. 
\system\ leverages an online learning agent that predicts the required resource configuration (CPU and memory) for each invocation to meet the user-specified SLO, given \emph{the characteristics of the input and function semantics}. 
%\system to (1) dynamically allocate resources per function invocation \emph{based on characteristics of the input and function semantics}, and (2) \emph{decouples different resource types}.
%{\system} removes the need for developers to specify a memory limit and leverages an online, cost-sensitive multi-class classification algorithm to predict the minimum amount resources (CPU, memory) to meet an \emph{invocation's} SLO.

A critical challenge to \system's delayed decision-making is the potential of increasing cold-starts. \neeraja{add a clause here tox``` this sentence explaining why ALAP may increase cold-starts.}
To mitigate such overheads, %{\system} inherently introduces with delayed decision making, 
we design \system's Scheduler that %tracks the sizes of all warm containers in the system and 
prioritizes routing invocations to perfectly sized containers that are warm. 
In case an instance of a desired size isn't available, \system's scheduler directs the invocation to a larger container that is warm, and 
to aid future invocations, launches the creation of perfectly sized containers in the background (taking it off the critical path). % if the invocation is routed to a larger container.
In doing so, the {\system} Scheduler reduces cold starts overheads while still ensuring high resource utilization. 

\noindent\textbf{Implementation and Results: }
We build {\system} for Apache OpenWhisk ~\cite{ApacheOpenWhisk} a popular open-source serverless platform used in previous research.
We evaluate {\system} against three static baselines and three state-of-the-art systems using the Azure production trace []. 
\prasoon{Get exact results with numbers and put them here!}

\noindent\textbf{Contributions: }
In summary, our main contributions are:
\renewcommand\labelenumi{(\theenumi)}
\begin{enumerate}
    \item Characterization of 12 commonly deployed serverless functions to reveal the importance of accounting for input properties and function semantics when making resource allocation decisions.
    \item The design of {\system}, resource management framework that delays allocation decisions until invocation without introducing excessive cold start overheads.
    \item The implementation and detailed evaluation of {\system} against three state-of-the-art serverless systems showing the improving in SLO compliance and resource utilization. \neeraja{add that sentence about open-sourcing your system to foster future research.}
\end{enumerate}








%     




==> 7_1_baselines.tex <==
\subsection{Baselines}
\label{sec: eval-baselines}
% \kostis{Add references to the baselines.}
We compare {\system} to two static baselines and three state-of-the-art systems, summarized below:
\renewcommand\labelenumi{(\theenumi)}
\begin{enumerate}
    \setlength{\itemsep}{0pt}
    \setlength{\parskip}{0pt}
    \item \textbf{Static-\{Medium, Large\}}: Users often request simple static allocations, choosing a medium (12 vCPUs, 6GB memory) or large (20 vCPUs, 10GB memory) allocation per function. These static baselines use OpenWhisk's default resource management and scheduling policies (memory-centric invocation scheduling). 
    \item \textbf{Static Allocation Developer Tools (Parrotfish)}:
    External tools assist developers in determining the optimal allocation prior to function deployment.
    % Developers may use external tools to determine the optimal allocation for their function prior to deployment.
    We use Parrotfish as the state-of-the-art developer tool~\cite{ParrotFish}.
    We provide Parrotfish with two representative inputs (medium and large) per function and use its recommendation for all invocations on top of OpenWhisk.
    \item \textbf{Bayesian Optimization (Aquatope)}: Bayesian optimization (BO) is a popular technique used to improve resource allocations in cloud settings \cite{CherryPick, Aquatope, Bilal-Serverless}. Aquatope constructs noise and uncertainty-aware Bayesian neural networks per function to make resource allocation decisions\cite{Aquatope} \emph{per function}. Although Aquatope targets serverless workflows, we use Aquatope to make single-stage workflow resource allocations. Similar to Parrotfish, we supply Aquatope with the same two representative inputs to obtain predicted allocations and request the predicted allocation for all invocations of that function. For a fair comparison, we use {\system}'s Scheduler with Aquatope's resource allocations because Aquatope decouples resource types and hence the scheduler should consider subscription of the server CPU. This also enables us to accurately compare {\system}'s and Aquatope's resource allocation schemes.
    \item \textbf{Bin-Packing Solutions (Cypress)}: Cypress packs invocations within a container to reduce container provisioning.
    It makes dynamic, input-size aware resource allocations by leveraging linear regression to predict execution time of an invocation and uses its prediction to assign a batch size per invocation \cite{cypress}. It packs similarly-sized batches into the same container to minimize container provisioning. We implement Cypress's resource allocation policies and mechanisms on top of OpenWhisk. 
\end{enumerate}

==> 7_4_eval_server_util.tex <==
\subsection{Server Utilization}
\label{sec:eval-server-util}
\kostis{Candidate for removal for space reasons.}
\prasoon{Agreed, Neeraja what do you think?}

% We provide a brief summary of the aggregate server utilization achieved between {\system} and the baselines.

